Dynamics and bifurcations on the normally hyperbolic invariant manifold of a periodically driven system with rank-1 saddle

In chemical reactions, trajectories typically turn from reactants to products when crossing a dividing surface close to the normally hyperbolic invariant manifold (NHIM) given by the intersection of the stable and unstable manifolds of a rank-1 saddle. Trajectories started exactly on the NHIM in principle never leave this manifold when propagated forward or backward in time. This still holds for driven systems when the NHIM itself becomes time dependent. We investigate the dynamics on the NHIM for a periodically driven model system with two degrees of freedom by numerically stabilizing the motion. Using Poincar\'e surfaces of section we demonstrate the occurrence of structural changes of the dynamics, \emph{viz.}, bifurcations of periodic transition state (TS) trajectories when changing the amplitude and frequency of the external driving. In particular, periodic TS trajectories with the same period as the external driving but significantly different parameters---such as mean energy---compared to the ordinary TS trajectory can be created in a saddle-node bifurcation.

==> engnames.tex <==
%
% engnames.tex 20.12.2006
%
\makeatletter
\def\contentsname{Contents}
\def\notesname{Notes}
\def\partname{Part}
\def\tocname{Contents}
\def\lofname{List of Figures}
\def\lotname{List of Tables}
\def\refname{REFERENCES}
\def\indexname{Index}
\def\figurename{Fig.}
\def\figuresname{Figures}%
\def\tablename{Table}
\def\tablesname{Tables}%
\def\abstractname{Abstract}
\def\appendixesname{Appendixes}%
\def\appendixname{Appendix}%
\def\acknowledgmentsname{Acknowledgments}
\def\journalname{??}
\def\copyrightname{??}
\def\andname{and}
\def\@pacs@name{MSC2010~numbers:}%
\def\@ydk@name{“„Љ~}%
\def\@keywords@name{Keywords:}%
\def\ppname{pp}
\def\numbername{number}
\def\volumename{volume}
\def\Dated@name{dated: }%
\def\Received@name{received }%
\def\Revised@name{in final form,~}%
\def\Accepted@name{accepted }%
\def\Published@name{published }%
\def\Presented@name{}%
%! 08.11.2006
\def\proofname{Proof}
\def\theoremname{Theorem}
\def\lemmaname{Lemma}
\def\propositionname{Proposition}
\def\assertionname{Assertion}
\def\corollaryname{Corollary}
\def\conjecturename{Conjecture}
\def\definitionname{Definition}
\def\remarkname{Remark}
\def\examplename{Example}
%!!
\makeatother
% ‘Ўа®б бзҐвзЁЄ®ў
\makeatletter
\setcounter{teo}{0}
\setcounter{teon}{0}
\setcounter{lem}{0}
\setcounter{lemn}{0}
\setcounter{prp}{0}
\setcounter{prpn}{0}
\setcounter{ass}{0}
\setcounter{assn}{0}
\setcounter{cor}{0}
\setcounter{corn}{0}
\setcounter{hyp}{0}
\setcounter{hypn}{0}
\setcounter{proof}{0}
\setcounter{proofn}{0}
\setcounter{exa}{0}
\setcounter{exan}{0}
\setcounter{dfn}{0}
\setcounter{dfnn}{0}
\setcounter{rem}{0}
\setcounter{remn}{0}
\setcounter{problem}{0}
\setcounter{problemn}{0}
\setcounter{notat}{0}
\setcounter{notatn}{0}
\makeatother
\endinput


==> jpack_e.tex <==
%%
%% This is file  `jpack_e.tex',  Strelkov S.A.  20.12.2006
%%
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsfonts}
%\usepackage{oldlfont} %%% Љ®­д«ЁЄвгҐв б bm.sty
\usepackage{mathtext}
\usepackage[T2A,OT1]{fontenc}
\usepackage[cp1251]{inputenc}
\usepackage[russian,english]{babel}
%\usepackage{literat}
\usepackage{pifont}
\usepackage{bm}
\usepackage{array}
\usepackage{dcolumn}
\usepackage{hhline}
\usepackage{multirow}
\usepackage{graphicx}
\usepackage{epsfig,color}
\usepackage{rotating}
\usepackage{srcltx_p}
\usepackage{calc}
\usepackage{tabularx}
\usepackage{afterpage}
\usepackage{ifthen}
\usepackage{caption2n}
\usepackage{substr}
%\usepackage{minitoc} 
\usepackage{psfrag}
\usepackage[all]{xy}
\usepackage{mathrsfs}
%\usepackage{supertabular}
\RequirePackage{soul}
\RequirePackage[amsmath]{ntheorem}
\RequirePackage{verbatim}
%
\theoremseparator{.}
\theoremindent 0pt
\theorempreskipamount 6pt plus2pt minus2pt
\theorempostskipamount 6pt plus2pt minus2pt
%
\RequirePackage{enumerate}
\makeatletter
\setcaptionwidth{\linewidth}
\renewcommand{\captionlabeldelim}{.~}
\renewcommand{\captionlabelfont}{\bfseries}
\renewcommand{\captionfont}{\footnotesize}
\renewcommand \thefigure{\@arabic\c@figure}
\renewcommand \thetable{\@arabic\c@table}
\renewcommand{\arraystretch}{1.5}
\setlength{\extrarowheight}{2pt}
\setlength{\extratabsurround}{2pt}
%%% Љ Є ў YADR.CLS
\renewcommand{\topfraction}{.90}
\renewcommand{\dbltopfraction}{.90}
\renewcommand{\bottomfraction}{.90}
\renewcommand{\textfraction}{0.10}
\renewcommand{\floatpagefraction}{0.90}
\renewcommand{\dblfloatpagefraction}{0.90}
\setcounter{topnumber}{4}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{6}
%
\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\let\PBS=\PreserveBackslash
\def\settabpars#1#2#3{\vskip#1mm \tabcolsep=#2pt \def\arraystretch{#3}}
\newdimen\tabwidth\newdimen\tbwdth
\newcommand{\stretchtab}[2][1.0]{\setbox0=\hbox{\tabcolsep=0sp\ignorespaces#2}
          \setbox1=\hbox{\tabcolsep=1sp\ignorespaces#2}
          \tabwidth=#1\hsize \advance\tabwidth by -\wd0
          %\multiply\tabwidth by 1
          \tbwdth=\wd1\advance\tbwdth by -\wd0
          \divide\tabwidth by \tbwdth
          \tabcolsep=\tabwidth #2}
\newcommand\figcaption{\def\@captype{figure}\caption}
% 26.07.2006 \newcommand\tabcaption{\def\@captype{table}\caption}
\newcommand\tabcaption{\let\captionfont\small\def\@captype{table}\caption}
\renewcommand*\caption@@@normal{%
\parfillskip0pt plus 2fil%
  \caption@label\captiontext\par}
\newcaptionstyle{nonumber}{%
  \usecaptionmargin%
  \captionfont%
  \onelinecaption%
    {{\parbox[t]{\realcaptionwidth}{\parfillskip0pt plus 2fil\captiontext}}}%
    {\parfillskip0pt plus 2fil\captiontext}
}%
\newcommand{\commes}[1]{#1}
%\newcommand{\commes}[1]{\relax}
\def\place@bibnumber@inl#1{#1.}%
\flushbottom
\def\refitem#1{\relax}
%\def\refitem#1{\ifthenelse{\boolean{hmode}}{\protect\newline{}}{}\textbackslash{}refitem\{\hbox{\bfseries{}\itshape{}#1}\}\ifthenelse{\boolean{hmode}}{\protect\linebreak{}}{}}

\def\qedsymbol{\square}
\def\qed{\ifmmode\let\next\eqnqed\else
    \let\next\textqed\fi\next}
\def\eqnqed{\relax\eqno{\raisebox{-2mm}{\qedsymbol}}\ignorespaces}
\def\textqed{{\unskip\nobreak\hfil\penalty50\hskip1em\null\nobreak\hfil
    $\qedsymbol$\parfillskip\z@\finalhyphendemerits0\smallbreak\par}}
\def\p@subsubsection{}
\def\p@subsection{}
\def\p@section{}
\let\mtcSfont=\mtcSSfont
\def\l@section#1#2{%
 \addpenalty{1000}%
 \addvspace{0.4em plus 5\p@}%
 \@tempdima 2em %
 \begingroup\leftskip=-2em
  \parindent \z@ \rightskip \@tocrmarg
  \parfillskip -\rightskip
  \leavevmode %
  \advance\leftskip\@tempdima %
  \hskip -2em %
  #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\nopagebreak\par
 \endgroup
}%
\def\l@subsection#1#2{%
 \addpenalty{2000}%
 \addvspace{0em plus 1\p@}%
 \@tempdima=3em %
 \begingroup
  \leftskip=0em
  \parindent 0em \rightskip \@tocrmarg
  \parfillskip -\rightskip
  \leavevmode
  \advance\leftskip\@tempdima %
  \hskip -\leftskip %
  #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\nopagebreak\par
 \endgroup
}%
%\def\l@subsection{\@dottedtocline{2}{0em}{2.5em}}
\def\theequation{\arabic{section}.\arabic{equation}}
\@addtoreset{equation}{section}

\gdef\th@nonumberplain{%
  \def\@begintheorem##1##2{%
      \item[\hskip\labelsep \theorem@headerfont ##1.]}%
  \def\@opargbegintheorem##1##2##3{%
     \item[\hskip\labelsep \theorem@headerfont ##1\ {\upshape(}##3\/{\upshape)}.]}}

\renewcommand{\labelenumi}{$\theenumi.$}
\def\const{{\rm const}}

\makeatother
\endinput


==> maikdoi.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%             This is maikdoi.tex  V 1.2 22.10.2009
%
% ЋЈа ­ЁзҐ­ЁҐ: ¬®¦­® а Ў®в вм в®«мЄ® б ISSN б®бв®пйЁ¬ Ё§ жЁда;
%              ¬®¦­® § ¤ ў вм \JournalISSNCode(1234-567X)
%              Ё«Ё \JournalCode(X2345671); ­Ґв Їа®ўҐаЄЁ Є®­ва®«м­®© бг¬¬л ISSN.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\ProvidesFile{maikdoi.tex}
              [2009/10/23 v1.2
       add-on for MAIK document class revtex4n]
\typeout{revtex4n Class enhancement: maikdoi.tex for DOI}
%
\makeatletter
%
\def\JournalISSNnumber#1#2#3#4#5#6#7#8#9\@fin{\gdef\@JournalISSNnumber{#1#2#3#4#6#7#8#9}}
\expandafter\JournalISSNnumber\@JournalISSNCode\@fin
\typeout{JournalISSNnumber=\@JournalISSNnumber}
% macros to get and set the basic informations
%\def\journalnumber#1{\xdef\journ@lnumber{\padt@eight@digits{#1}}%
\def\journalnumber#1{\xdef\journ@lnumber{#1}%
%\checksize{journalnumber}8\journ@lnumber{99999999}%
}%
%\let\journ@lnumber=\empty
%
\def\ShortYear#1#2#3#4\@fin{\gdef\@ShortYear{#3#4}}
\expandafter\ShortYear\@TransYearOfIssue\@fin
\typeout{ShortYear=\@ShortYear}
\def\DOIyear#1{\xdef\DOI@year{\padt@two@digits{#1}}\checksize{DOIyear}2\DOI@year{99}}%
%
\def\DOIpsniy#1{\xdef\DOI@psniy{\padt@two@digits{#1}}% psniy - PublicationSerialNumberInYear
\checksize{DOIpsniy}2\DOI@psniy{99}}%
%
\def\DOIartnumber#1{\xdef\DOI@artnumber{\padt@three@digits{#1}}%
\checksize{DOIartnumber}3\DOI@artnumber{999}}
\def\DOI@artnumber{0}
%
\def\doitext#1{\xdef\doit@xtpref{#1}}
%
% a helpful hand of macros
\newif\if@wrongformat \@wrongformatfalse
%
\def\checksize#1#2#3#4{\ifnum#3>#4\PackageError{DOI2module}%
{Numeric value for "#1" to large!\MessageBreak
"#3" specified, but only #2 digits allowed}{Check your input!}
\@wrongformattrue \fi}
%
\newcount\modarg
\newcount\modmod
\newcount\tmp
\def\modulo{\tmp=\modarg\divide\modarg by\modmod\multiply\modarg
by\modmod\multiply\modarg by-1\global\advance\modarg by\tmp}
%
\def\padt@two@digits#1{\ifnum#1<10 0\fi\number#1}%
\def\padt@three@digits#1{\ifnum#1<100 0\fi%
\ifnum#1<10 0\fi\number#1}%
\def\padt@four@digits#1{\ifnum#1<1000 0\fi\ifnum#1<100 0\fi%
\ifnum#1<10 0\fi\number#1}%
\def\padt@five@digits#1{\ifnum#1<10000 0\fi\ifnum#1<1000 0\fi\ifnum#1<100 0\fi%
\ifnum#1<10 0\fi\number#1}%
\def\padt@eight@digits#1{\ifnum#1<1000000 0\fi\ifnum#1<1000000 0\fi\ifnum#1<100000 0%
\fi\ifnum#1<10000 0\fi\ifnum#1<1000 0\fi\ifnum#1<100 0\fi%
\ifnum#1<10 0\fi\number#1}%
%\def\setjahr#1{\xdef\jahr{#1}}
% @pii_digits_weights = (53,47,43,41,37,31,29,23,19,17,13,7,5,3,2);
\def\teilissn#1#2#3#4#5#6#7#8\@fin{%
\if#1X\modarg=10\relax\else\modarg=#1\relax\fi\multiply\modarg by53\advance\tmp by\modarg%
\if#2X\modarg=10\relax\else\modarg=#2\relax\fi\multiply\modarg by47\advance\tmp by\modarg%
\if#3X\modarg=10\relax\else\modarg=#3\relax\fi\multiply\modarg by43\advance\tmp by\modarg%
\if#4X\modarg=10\relax\else\modarg=#4\relax\fi\multiply\modarg by41\advance\tmp by\modarg%
\if#5X\modarg=10\relax\else\modarg=#5\relax\fi\multiply\modarg by37\advance\tmp by\modarg%
\if#6X\modarg=10\relax\else\modarg=#6\relax\fi\multiply\modarg by31\advance\tmp by\modarg%
\if#7X\modarg=10\relax\else\modarg=#7\relax\fi\multiply\modarg by29\advance\tmp by\modarg%
\if#8X\modarg=10\relax\else\modarg=#8\relax\fi\multiply\modarg by23\advance\tmp by\modarg}
\def\teilyear#1#2\@fin{%
\modarg=#1\relax\multiply\modarg by19\advance\tmp by\modarg%
\modarg=#2\relax\multiply\modarg by17\advance\tmp by\modarg}
\def\teilpsniy#1#2\@fin{%
\modarg=#1\relax\multiply\modarg by13\advance\tmp by\modarg%
\modarg=#2\relax\multiply\modarg by7\advance\tmp by\modarg}
\def\teilartnumber#1#2#3\@fin{%
\modarg=#1\relax\multiply\modarg by5\advance\tmp by\modarg%
\modarg=#2\relax\multiply\modarg by3\advance\tmp by\modarg%
\modarg=#3\relax\multiply\modarg by2\advance\tmp by\modarg}
%
% check for all required elements
\def\checkrequirements{
\if!\journ@lnumber!\typein[\answer]{^^JMissing 5-digit
journalnumber for the DOI, please specify:}\journalnumber\answer\fi
%
\ifnum\OF@year=0\typein[\answer]{^^JMissing 4-digit year for the OF
date, please specify:}\OFyear\answer\fi
%
\ifnum\DOI@year=0\typein[\answer]{^^JMissing 4-digit year for the DOI,
please specify:}\DOIyear\answer\fi
{\modarg=\DOI@year\relax\modmod=1000\relax\modulo
\expandafter\setjahr{\padt@three@digits\modarg}}
%
\if!\the\DOI@msnr!\typein[\answer]{^^JMissing 4-digit
manuscript number for the DOI, please specify:}\DOImsnr\answer\fi}
%
% make the package verbose
\def\showDOIargs{%
\typeout{^^JList of arguments for this DOI2 generation
^^J==========================================
^^JDOI-prefix :\space\maikpraefix
^^JISSN number:\space\journ@lnumber
^^JDOI-year\space\space\space:\space\DOI@year
^^JIn-Year-No.:\space\DOI@psniy
^^JArticle-No.:\space\DOI@artnumber
^^J==========================================}}
%
% perform the calculation
\def\DOIt{\if@wrongformat
   \typeout{Wrong format of at least one required value,^^Jno
            DOI could be generated.^^J}%
\else
   \edef\doit@xtcode{%
   \maikpraefix\journ@lnumber\DOI@year\DOI@psniy\DOI@artnumber}%
   \tmp=0\relax%
   \expandafter\teilissn\journ@lnumber\@fin%
   \expandafter\teilyear\DOI@year\@fin%
   \expandafter\teilpsniy\DOI@psniy\@fin%
   \expandafter\teilartnumber\DOI@artnumber\@fin%
   \modarg=\tmp\modmod=11\relax\modulo
   \ifnum\modarg<10\edef\checksum{\the\modarg}\else\edef\checksum{X}%
   \fi
   \edef\doit@xtcode{\doit@xtcode\checksum}
   \edef\doit@xt{\doit@xtpref\doit@xtcode}
   \showDOIargs
   \typeout{Calculated DOI:\space\space\doit@xtcode
   ^^J^^JVerbose:^^J\doit@xt^^J}
\fi
}
%
% set the defaults - the basics at least
%\def\springerpraefix{10.1007/s}
%!\def\maikpraefix{10.1134/S}
\doitext{\relax}%
%! 22.10.2009
\def\OnlineFirstDOI#1#2{\def\doit@xtcode{#1}%
\def\@onlinefirstdoi{#1}%
\def\@onlinefirstfilename{#2}%
\@booleantrue\onlinefirstdoi@sw%
\ifthenelse{\equal{\@nameincfi}{#2}}{%
\addtocounter{doiartnumber}{-\@ne}
}%
{\class@err{ ^^J^^J
\space\space \noexpand\OnlineFirstDOI{#1}{#2}^^J
\space\space Name Online First file:  #2^^J
\space\space Includepaper file name: \@nameincfi^^J
\space\space Not equal}%
}%
}%
%!!
%
\journalnumber{\@JournalISSNnumber}
\typeout{journalnumber=\journ@lnumber}
\DOIyear{\@ShortYear}
\typeout{DOIyear=\DOI@year}
\DOIpsniy{\@PublicationSerialNumberInYear}
\typeout{DOIpsniy=\DOI@psniy}
\makeatother
\endinput
%% End of file `maik.doi'


==> optn.tex <==
%%
%% This is file `optn.tex',  Strelkov S.A.  30.01.2002
%%
\begingroup
\catcode`\+\active\gdef+{\mathchar8235\nobreak\discretionary{}{\usefont{OT1}{cmr}{m}{n}\char43}{}}
\catcode`\-\active\gdef-{\mathchar8704\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char0}{}}
\catcode`\=\active\gdef={\mathchar12349\nobreak\discretionary{}{\usefont{OT1}{cmr}{m}{n}\char61}{}}
\endgroup
\def\cdot{\mathchar8705\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char1}{}}
\def\times{\mathchar8706\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char2}{}}
\mathcode`\==32768
\mathcode`\+=32768
\mathcode`\-=32768
% Љ« бб ¬ вҐ¬ вЁзҐбЄ®Ј® бЁ¬ў®«  TeXBook бвао 185-186
% 2 --- ЃЁ­ а­л© ®ЇҐа в®а
% 3 --- Ћв­®иҐ­ЁҐ
% <\equiv =\mathchar"3211>
\def \equiv   {\mathchar8721\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char17}{}}% "2211
% A.2.2~ЃЁ­ а­лҐ ®в­®иҐ­Ёп~LaTeX'a
% <\subseteq =\mathchar"3212>
\def \subseteq{\mathchar8722\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char18}{}} % "2222
% <\supseteq =\mathchar"3213>
\def \supseteq{\mathchar8723\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char19}{}}
\def \leq     {\mathchar8724\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char20}{}}
\def \geq     {\mathchar8725\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char21}{}}
\def \sim     {\mathchar8728\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char24}{}}
\def \approx  {\mathchar8729\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char25}{}}
\def \subset  {\mathchar8730\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char26}{}}
\def \supset  {\mathchar8731\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char27}{}}
\def \ll      {\mathchar8732\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char28}{}}
\def \gg      {\mathchar8733\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char29}{}}
\def \pm      {\mathchar8710\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char6}{}}
\def \mp      {\mathchar8711\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char7}{}}
\def \in      {\mathchar8754\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char50}{}}
\def \ni      {\mathchar8755\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char51}{}}
% ‘¬. TeXBook бва. 510-511
% ЌҐЄ®в®алҐ бЁ¬ў®«л Ё¬Ґов  «мвҐа­ вЁў­лҐ Ё¬Ґ­ , Є®в®алҐ в Є иЁа®Є® ЁбЇ®«м§говбп,
% зв® plain TeX Ё¬ҐҐв ¤«п ­Ёе Ї® ¤ўҐ Ё«Ё Ў®«ҐҐ Є®¬ ­¤­лҐ Ї®б«Ґ¤®ў вҐ«м­®бвЁ:
% \ne Ё«Ё \neq (в® ¦Ґ, зв® \not=)
% \le          (в® ¦Ґ, зв® \leq)
% \ge          (в® ¦Ґ, зв® \geq)
% (в® ¦Ґ, зв® )
% (в® ¦Ґ, зв® )
% (в® ¦Ґ, зв® )
%<\prec =\mathchar"321E>
\def \prec    {\mathchar"321E\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"1E}{}}
%<\succ =\mathchar"321F>
\def \succ    {\mathchar"321F\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"1F}{}}
%<\preceq =\mathchar"3216>
\def \preceq  {\mathchar"3216\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"16}{}}
%<\succeq =\mathchar"3217>
\def \succeq  {\mathchar"3217\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"17}{}}
%<\simeq =\mathchar"3227>
\def \simeq  {\mathchar"3227\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"27}{}}
%<\cong =macro:->\mathrel {\mathpalette \@vereq \sim }>
%<\doteq =\long macro:->\DOTSB \mathrel {\mathop {\kern 0pt =}\limits ^{\textstyle .}}>
%<\sqsubseteq =\mathchar"3276>
\def \sqsubseteq {\mathchar"3276\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"76}{}}
%<\sqsupseteq =\mathchar"3277>
\def \sqsupseteq {\mathchar"3277\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"77}{}}
%<\smile =\mathchar"315E>
\def \smile   {\mathchar"315E\nobreak\discretionary{}{\usefont{OML}{cmm}{m}{n}\char"5E}{}}
%<\frown =\mathchar"315F>
\def \frown   {\mathchar"315F\nobreak\discretionary{}{\usefont{OML}{cmm}{m}{n}\char"5F}{}}
%<\perp =\mathchar"323F>
\def \perp    {\mathchar"323F\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"3F}{}}
%<\models =macro:->\mathrel {|}\joinrel \Relbar >
%<\mid =\mathchar"326A>
\def \mid     {\mathchar"326A\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"6A}{}}
%<\parallel =\mathchar"326B>
\def \parallel {\mathchar"326B\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"6B}{}}
%<\vdash =\mathchar"3260>
\def \vdash  {\mathchar"3260\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"60}{}}
%<\dashv =\mathchar"3261>
\def \dashv  {\mathchar"3261\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"61}{}}
%<\propto =\mathchar"322F>
\def \propto  {\mathchar"322F\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"2F}{}}
%<\asymp =\mathchar"3210>
\def \asymp  {\mathchar"3210\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"10}{}}
% latexsym
%<\sqsubset =\mathchar"3440>
\def \sqsubset {\mathchar"3440\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"40}{}}
%<\sqsupset =\mathchar"3441>
\def \sqsupset {\mathchar"3441\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"41}{}}
% A.2.2~ЃЁ­ а­лҐ ®в­®иҐ­Ёп~AMS
%<\leqslant =\mathchar"3436>
\def \leqslant {\mathchar"3436\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"36}{}}
%<\geqslant =\mathchar"343E>
\def \geqslant {\mathchar"343E\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"3E}{}}
%<\eqslantless =\mathchar"3430>
\def \eqslantless {\mathchar"3430\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"30}{}}
%<\eqslantgtr =\mathchar"3431>
\def \eqslantgtr {\mathchar"3431\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"31}{}}
%<\lesssim =\mathchar"342E>
%\def \lessim {\mathchar"342E\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"2E}{}}
%<\gtrsim =\mathchar"3426>
\def \gtrsim {\mathchar"3426\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"26}{}}
%<\lll =\mathchar"346E>
\def \lll {\mathchar"346E\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"6E}{}}
%<\ggg =\mathchar"346F>
\def \ggg {\mathchar"346F\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"6F}{}}
%<\lessgtr =\mathchar"3437>
\def \lessgtr {\mathchar"3437\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"37}{}}
%<\gtrless =\mathchar"343F>
\def \gtrless {\mathchar"343F\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"3F}{}}
%<\doteqdot =\mathchar"342B>
\def \doteqdot {\mathchar"342B\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"2B}{}}
%<\eqcirc =\mathchar"3450>
\def \eqcirc {\mathchar"3450\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"50}{}}
%<\circeq =\mathchar"3424>
\def \circeq {\mathchar"3424\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"24}{}}
%<\triangleq =\mathchar"342C>
\def \triangleq {\mathchar"342C\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"2C}{}}
%<\risingdotseq =\mathchar"343A>
\def \risingdotseq {\mathchar"343A\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"3A}{}}
%<\fallingdotseq =\mathchar"343B>
\def \fallingdotseq {\mathchar"343B\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"3B}{}}
%<\subseteqq =\mathchar"346A>
\def \subseteqq {\mathchar"346A\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"6A}{}}
%<\supseteqq =\mathchar"346B>
\def \supseteqq {\mathchar"346B\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"6B}{}}
%<\vartriangleleft =\mathchar"3443>
\def \vartriangleleft {\mathchar"3443\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"43}{}}
%<\vartriangleright =\mathchar"3442>
\def \vartriangleright {\mathchar"3442\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"42}{}}
% A.2.3~ЃЁ­ а­лҐ ®в­®иҐ­Ёп~AMS~б~®ваЁж ­ЁҐ¬
\def \neq      {\hbox{\text{\kern0.3em{\usefont{OMS}{cmsy}{m}{n}\char54}=}\kern0.3em}\nobreak\discretionary{}{{\usefont{OMS}{cmsy}{m}{n}\char54}=\kern0.3em}{}}
\let\ne=\neq
% <\nless =\mathchar"3504>
\def \nless   {\mathchar"3504\nobreak\discretionary{}{{\usefont{U}{msb}{m}{n}\char"04}}{}}
%<\in =\mathchar"3232>
%<\notin =macro:->\mathrel {\m@th \mathpalette \c@ncel \in }>
%<\nparallel =\mathchar"352C>
\def \nparallel {\mathchar"352C\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"2C}{}}
%<\nsubseteq =\mathchar"352A>
\def \nsubseteq {\mathchar"352A\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"2A}{}}
%<\nsupseteq =\mathchar"352B>
\def \nsupseteq {\mathchar"352B\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"2B}{}}
% A.3~ЃЁ­ а­лҐ~®ЇҐа жЁЁ
%<\circ =\mathchar"220E>
\def \circ {\mathchar"220E\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"0E}{}}
%<\bigcirc =\mathchar"220D>
\def \bigcirc {\mathchar"220D\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"0D}{}}
%<\div =\mathchar"2204>
\def \div {\mathchar"2204\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"04}{}}
%<\diamond =\mathchar"2205>
\def \diamond {\mathchar"2205\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"05}{}}
%<\ast =\mathchar"2203>
\def \ast {\mathchar"2203\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"03}{}}
%<\star =\mathchar"213F>
\def \star {\mathchar"213F\nobreak\discretionary{}{\usefont{OML}{cmm}{m}{n}\char"3F}{}}
%<\cap =\mathchar"225C>
\def \cap {\mathchar"225C\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"5C}{}}
%<\cup =\mathchar"225B>
\def \cup {\mathchar"225B\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"5B}{}}
%<\sqcap =\mathchar"2275>
\def \sqcap {\mathchar"2275\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"75}{}}
%<\sqcup =\mathchar"2274>
\def \sqcup {\mathchar"2274\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"74}{}}
%<\wedge =\mathchar"225E>
\def \wedge {\mathchar"225E\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"5E}{}}
%<\vee =\mathchar"225F>
\def \vee {\mathchar"225F\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"5F}{}}
%<\oplus =\mathchar"2208>
\def \oplus {\mathchar"2208\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"08}{}}
%<\ominus =\mathchar"2209>
\def \ominus {\mathchar"2209\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"09}{}}
%<\otimes =\mathchar"220A>
\def \otimes {\mathchar"220A\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"0A}{}}
%<\odot =\mathchar"220C>
\def \odot {\mathchar"220C\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"0C}{}}
%<\Cap =\mathchar"2465>
\def \Cap {\mathchar"2465\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"65}{}}
%<\Cup =\mathchar"2464>
\def \Cup {\mathchar"2464\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"64}{}}
% A.4~‘ваҐ«ЄЁ
%<\leftarrow =\mathchar"3220>
\def \leftarrow  {\mathchar"3220\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"20}{}}
%<\rightarrow =\mathchar"3221>
\def \rightarrow  {\mathchar"3221\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"21}{}}
%<\to =\mathchar"3221>
\def \to  {\mathchar"3221\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"21}{}}
%<\longleftarrow =\long macro:->\DOTSB \leftarrow \protect \joinrel \protect \relbar >
%<\longrightarrow =\long macro:->\DOTSB \protect \relbar \protect \joinrel \rightarrow >
%<\Leftarrow =\mathchar"3228>
\def \Leftarrow  {\mathchar"3228\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"28}{}}
%<\Rightarrow =\mathchar"3229>
\def \Rightarrow  {\mathchar"3229\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"29}{}}
%<\Longleftarrow =\long macro:->\DOTSB \Leftarrow \protect \joinrel \protect \Relbar >
%<\Longrightarrow =\long macro:->\DOTSB \protect \Relbar \protect \joinrel \Rightarrow >
%<\leftrightarrow =\mathchar"3224>
\def \leftrightarrow  {\mathchar"3224\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"24}{}}
%<\longleftrightarrow =\long macro:->\DOTSB \leftarrow \joinrel \rightarrow >
%<\Leftrightarrow =\mathchar"322C>
\def \Leftrightarrow  {\mathchar"322C\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"2C}{}}
%<\Longleftrightarrow =\long macro:->\DOTSB \Leftarrow \joinrel \Rightarrow >
%<\uparrow =macro:->\delimiter "3222378 >
%<\downarrow =macro:->\delimiter "3223379 >
%<\Uparrow =macro:->\delimiter "322A37E >
%<\Downarrow =macro:->\delimiter "322B37F >
%<\updownarrow =macro:->\delimiter "326C33F >
%<\Updownarrow =macro:->\delimiter "326D377 >
%<\leftleftarrows =\mathchar"3412>
\def \leftleftarrows {\mathchar"3412\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"12}{}}
%<\rightrightarrows =\mathchar"3413>
\def \rightrightarrows {\mathchar"3413\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"13}{}}
%<\leftrightarrows =\mathchar"341C>
\def \leftrightarrows {\mathchar"341C\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"1C}{}}
%<\rightleftarrows =\mathchar"341D>
\def \rightleftarrows {\mathchar"341D\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"1D}{}}
%<\upuparrows =\mathchar"3414>
\def \upuparrows {\mathchar"3414\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"14}{}}
%<\downdownarrows =\mathchar"3415>
\def \downdownarrows {\mathchar"3415\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"15}{}}
%<\nLeftarrow =\mathchar"353A>
\def \nLeftarrow {\mathchar"353A\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"3A}{}}
%<\nRightarrow =\mathchar"353B>
\def \nRightarrow {\mathchar"353B\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"3B}{}}
\endinput
%\DeclareFontEncoding{OML}{}{}
%\DeclareFontEncoding{OMS}{}{}
%\DeclareFontEncoding{OMX}{}{}
%\DeclareFontEncoding{U}{}{\noaccents@}
%\DeclareFontSubstitution{OML}{cmm}{m}{it}
%\DeclareFontSubstitution{OMS}{cmsy}{m}{n}
%\DeclareFontSubstitution{OMX}{cmex}{m}{n}
%\DeclareFontSubstitution{U}{cmr}{m}{n}

